ChemActor: Enhancing Automated Extraction of Chemical Synthesis Actions with LLM-Generated Data

With the increasing interest in robotic synthesis in the context of organic chemistry, the automated extraction of chemical procedures from literature is critical. However, this task remains challenging due to the inherent ambiguity of chemical language and the high cost of human annotation required for developing reliable computer-aided extraction protocols. Here, we present ChemActor, a fully fine-tuned large language model (LLM), as a chemical executor to convert between unstructured experimental procedures and structured action sequences. We propose a sequential LLM-generated data framework to address the challenges of insufficient and low-quality annotated data. This framework integrates a data selection module that selects data based on distribution divergence, with a general-purpose LLM, to generate machine-executable actions from a single molecule input. Additionally, we introduce a novel multi-round LLMs circle review metric, which reflects the model's advanced understanding of chemical experimental procedures. Extensive experiments on reaction-to-description (R2D) and description-to-action (D2A) tasks demonstrate that ChemActor, augmented by LLM-generated data, achieves state-of-the-art performance, outperforming the baseline model by 10%. The code is available at: https://github.com/Zhanghahah/ChemActor.

==> latex/table/badcase.tex <==
\begin{table*}[]
\centering
% \setlength{\belowcaptionskip}{-0.5cm}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{@{}c|l|l|l@{}}
\toprule
            & \multicolumn{1}{c|}{\textbf{Long-distance information.}}                                                                                                                                                                                                                                                                                                              & \multicolumn{1}{c|}{\textbf{Evidence uncertainty.}}                                                                                                                                                                                                                                                                                      & \multicolumn{1}{c}{\textbf{Concept confusion.}}                                                                                                                                                                                                                                                                                                                                        \\ \midrule
\textbf{Question}  & Who did Iga Swiatek defeat to win the Qatar Open 2022?                                                                                                                                                                                                                                                                                                                & What is the name of Apple's headset?                                                                                                                                                                                                                                                                                                   & What was Tesla's revenue in Q1 2022?                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
\textbf{Answer}    & \textbf{Anett Kontaveit}                                                                                                                                                                                                                                                                                                                                              & \textbf{Vision Pro}                                                                                                                                                                                                                                                                                                                    & \textbf{18.76 billion}                                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
\textbf{Documents} & \begin{tabular}[c]{@{}l@{}}\emph{Positive document}\\ In February, Swiatek entered into the \textcolor{blue}{Qatar Open} ...\\ In the final, she won ... \textbf{\textcolor{blue}{Anett Kontaveit}} ...\\ \\ \emph{Negative document}\\ This time, she defeated \textcolor{red}{Ons Jabeur} 6-2, 7-6(5) to win\\ the \textcolor{red}{2022 US Open}, ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}\emph{Positive document}\\ Apple (AAPL.O) on Monday unveiled a costly\\ augmented-reality \textcolor{blue}{headset} called the \textbf{\textcolor{blue}{Vision Pro}} ...\\ \\ \emph{Negative document}\\ ... is what Gurman believes will be called \\ \textcolor{red}{Apple Reality Pro}. ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}\emph{Positive document}\\ \textcolor{blue}{Tesla, Inc. (TSLA) reported Q1 FY 2022} earnings results\\ ... detailed revenues of \$\textbf{\textcolor{blue}{18.76 billion}} ...\\ \\ \emph{Negative document}\\ ...\textcolor{blue}{first-quarter earnings for 2022} ...\\ ...\textcolor{red}{Automotive revenue} reached \$\textcolor{red}{16.86 billion}...\end{tabular} \\ \midrule
\textbf{Responses} & \begin{tabular}[c]{@{}l@{}}Iga Swiatek defeated \textcolor{red}{Ons Jabeur} in the \textcolor{red}{second round}\\  of the Qatar Open 2022 to win the tournament.\end{tabular}                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}According to the document, the name of Apple's\\ headset is \textcolor{red}{Apple Reality Pro}.\end{tabular}                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}According to the financial results provided in the article,\\ Tesla's revenue in Q1 2022 was \$\textcolor{red}{16.86 billion}.\end{tabular}                                                                                                                                                                                                                               \\ \bottomrule
\end{tabular}}
\caption{Error cases of noise robustness, and only one positive document and one negative document are shown. The responses are generated by ChatGLM2-6B. The blue text indicates the matching parts between the document and the question or answer, while the red text highlights the non-matching parts.}
\label{tab:case1}
\end{table*}

==> latex/table/retro.tex <==
% retrosynthesis prediction performance
\begin{table}[h!]
{
\centering
% \renewcommand{\arraystretch}{1.1}
% \caption{Top-$k$ accuracy for retrosynthesis prediction tasks on USPTO-50K (reaction class unknown). * indicates the model with SMILES augmentation. Best performance is in \textbf{bold}.}\label{tab:retro-res}
\caption{Experiment \textcolor{red}{results} for retrosynthesis prediction tasks on USPTO-50k (reaction class unknown) dataset. The best performance is in \textbf{bold}. * indicates the model with SMILES augmentation.}\label{tab:retro-res}
\resizebox{\columnwidth}{!}
{
\resizebox{0.55\textwidth}{!}{\begin{tabular}{lccc}
% \begin{tabular}{p{5.5cm} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering}}
% \resizebox{0.55\textwidth}
\bottomrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c} {\textbf{Top-$k$ accuracy (\%)}} \\ 
\cline{2-4} 
\multicolumn{1}{c}{} & 1 & 3 & 5\\ 
\hline
% \vspace{0.2cm}
\textit{Template-based models} & & & \\ 
% \hline
% GLN~\cite{gln} &  52.5 & 69.0 & 75.6 \\
% LocalRetro~\cite{localretro} & 53.4 & 77.5 & 85.9 \\ 
$\mathcal {O} $-GNN~\cite{zhu2023mathcal} & 54.1 & 77.7 & 86 \\
RetroKNN~\cite{xie2023retrosynthesis} & \textbf{57.2}& \textbf{78.9}& \textbf{86.4}\\
\hline
\textit{Semi-template-based models} & & & \\ 
% \hline
% RetroXpert*~\cite{yan2020retroxpert} & 50.4 & 61.1 & 62.3\\
% G2G~\cite{shi2020graph2graph} & 48.9 & 67.6 & 72.5  \\
% GraphRetro~\cite{somnath2021graphretro} & 53.7 & 68.3 & 72.2\\
RetroPrime*~\cite{retroprime} & 51.4 & 70.8 & {74.0}\\ 
% MEGAN~\cite{megan} & 48.1 & 70.7  & 78.4  \\ 
G2Retro~\cite{Chen2023g2retro} & \textbf{54.1} &\textbf{74.1}&\textbf{81.2}\\
\hline
\textit{Template-free models} & & &\\ 
% \hline
% Transformer~\cite{vaswani2017attention} & 42.4 & 58.6 & 63.8\\
% SCROP~\cite{zheng2019predicting} & 43.7 & 60.0 & 65.2\\
% Tied Transformer~\cite{kim2021valid} & 47.1 & 67.1 & 73.1\\
% Aug. Transformer* \cite{tetko2020state}& 48.3 & - & 73.4\\
% GTA* \cite{GTA} & 51.1 & 67.6 & 74.8 \\
% Graph2SMILES~\cite{tu2022permutation} & {52.0} & 70.2 & 75.2\\
% Retroformer*~\cite{wan2022retroformer} & 53.2 & 71.1 & 76.6  \\ 
% RetroExplainer~\cite{wang2023retrosynthesis} & 57.7 & \textbf{79.2} & \textbf{84.8} \\
NAG2G~\cite{yao2024node} & 55.1 & 76.9 & 83.4 \\
% Chemma & \textbf{72.2} & \textbf{78.9} & \textbf{84.2}\\
Graph2Edits~\cite{zhong2023retrosynthesis} &  55.1 & 77.3 & 83.4 \\
G2GT*~\cite{lin2023g2gt} & 54.1 & 69.9 & 74.5 \\
UAlign*~\cite{zeng2024ualign} & 53.5 & 77.3 & 84.6 \\
ChemActor* & 72.2 & 78.3 & 84.2 \\
ChemActor*, w/g & \textbf{74.9} & \textbf{79.9} & \textbf{85.2} \\

\bottomrule
\end{tabular}
}
}

% \vspace{-5pt}
\end{table}
